Make-Your-Anchor: A Diffusion-based 2D Avatar Generation Framework

Despite the remarkable process of talking-head-based avatar-creating solutions, directly generating anchor-style videos with full-body motions remains challenging. In this study, we propose Make-Your-Anchor, a novel system necessitating only a one-minute video clip of an individual for training, subsequently enabling the automatic generation of anchor-style videos with precise torso and hand movements. Specifically, we finetune a proposed structure-guided diffusion model on input video to render 3D mesh conditions into human appearances. We adopt a two-stage training strategy for the diffusion model, effectively binding movements with specific appearances. To produce arbitrary long temporal video, we extend the 2D U-Net in the frame-wise diffusion model to a 3D style without additional training cost, and a simple yet effective batch-overlapped temporal denoising module is proposed to bypass the constraints on video length during inference. Finally, a novel identity-specific face enhancement module is introduced to improve the visual quality of facial regions in the output videos. Comparative experiments demonstrate the effectiveness and superiority of the system in terms of visual quality, temporal coherence, and identity preservation, outperforming SOTA diffusion/non-diffusion methods. Project page: \url{https://github.com/ICTMCG/Make-Your-Anchor}.

==> figure/512FE.tex <==
\begin{figure}[htp]
\vspace{-10px}
% \newcommand{\galleryfigurewidth}{0.10}
%     \begin{minipage}[t]{0.32\linewidth}
%         \includegraphics[width=\linewidth]{gifs/crossmotion/000005.png}
%     \end{minipage}
%     \begin{minipage}[t]{0.32\linewidth}
%         \includegraphics[width=\linewidth]{gifs/crossmotion/000282.png}
%     \end{minipage}
%     \begin{minipage}[t]{0.32\linewidth}
%         \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/crossmotion/000}{180}{210}
%     \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \includegraphics[width=\linewidth]{gifs/fullbody/000010.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \includegraphics[width=\linewidth]{gifs/fullbody/000176.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/fullbody/000}{281}{294}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \includegraphics[width=\linewidth]{gifs/perturb/000160.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \includegraphics[width=\linewidth]{gifs/perturb/000270.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/perturb/000}{074}{100}
    % \end{minipage}
    % \begin{subfigure}[t]{0.48\linewidth}
    %     \vspace{-15px}
    %     \subcaption*{\tiny (a) Cross-person motion. Left reference, right output.}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.24\linewidth}
    %     \vspace{-15px}
    %     \subcaption*{\tiny (b) Full-body Video.}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.24\linewidth}
    %     \vspace{-15px}
    %     \subcaption*{\tiny (c) Trained with SMPL perturbation.}
    % \end{subfigure}

    % \vspace{-4px}
    
    \begin{minipage}[t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{gifs/face/000007.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\linewidth}
        \includegraphics[width=\linewidth]{gifs/face/000017.png}
    \end{minipage}
    \begin{minipage}[t]{0.32\linewidth}
        \animategraphics[width=\linewidth,autoplay=True]{15}{gifs/face/0000}{03}{32}
    \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \includegraphics[width=\linewidth]{gifs/twostage/nopretrain/000007.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \includegraphics[width=\linewidth]{gifs/twostage/nopretrain/000069.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/twostage/nopretrain/0000}{76}{88}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \includegraphics[width=\linewidth]{gifs/twostage/alltrainonce/000007.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \includegraphics[width=\linewidth]{gifs/twostage/alltrainonce/000017.png}
    % \end{minipage}
    % \begin{minipage}[t]{0.07\linewidth}
    %     \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/twostage/alltrainonce/0000}{76}{88}
    % \end{minipage}
    % \begin{subfigure}[t]{0.48\linewidth}
    %     \vspace{-15px}
    %     \subcaption*{\tiny (d) Improved FE. Left 256px, right 512px.}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.24\linewidth}
    %     \vspace{-15px}
    %     \subcaption*{\tiny (e) Directly training video of target subject.}
    % \end{subfigure}
    % \begin{subfigure}[t]{0.24\linewidth}
    %     \vspace{-15px}
    %     \subcaption*{\tiny (f) Training target with all other subjects.}
    % \end{subfigure}


    % \begin{minipage}[t]{0.45\linewidth}
    %     \begin{minipage}[t]{0.3\linewidth}
    %         \includegraphics[width=\linewidth]{gifs/crossmotion/000005.png}
    %     \end{minipage}
    %     \begin{minipage}[t]{0.3\linewidth}
    %         \includegraphics[width=\linewidth]{gifs/crossmotion/000282.png}
    %     \end{minipage}
    %     \begin{minipage}[t]{0.3\linewidth}
    %         \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/crossmotion/000}{180}{210}
    %     \end{minipage}
    %     \begin{subfigure}[t]{\linewidth}
    %         \subcaption*{\tiny Cross-person motion. Left pose, right output.}
    %     \end{subfigure}
    %     \vspace{-15px}
    % \end{minipage}

    % \begin{minipage}[t]{0.45\linewidth}
    %     \begin{minipage}[t]{0.3\linewidth}
    %         \includegraphics[width=\linewidth]{gifs/face/000007.png}
    %     \end{minipage}
    %     \begin{minipage}[t]{0.3\linewidth}
    %         \includegraphics[width=\linewidth]{gifs/face/000017.png}
    %     \end{minipage}
    %     \begin{minipage}[t]{0.3\linewidth}
    %         \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/face/0000}{01}{34}
    %     \end{minipage}
    %     \begin{subfigure}[t]{\linewidth}
    %         \subcaption*{\tiny Improved FE. Left 256px, right 512px.}
    %     \end{subfigure}
    %     \vspace{-15px}
    % \end{minipage}


    % \begin{minipage}[t]{\galleryfigurewidth\linewidth}
    %     \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/twostage/ours/0000}{74}{90}
    % \end{minipage}
    % \begin{minipage}[t]{\galleryfigurewidth\linewidth}
    %     \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/twostage/nopretrain/0000}{74}{90}
    % \end{minipage}    
    % \begin{minipage}[t]{\galleryfigurewidth\linewidth}
    %     \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/twostage/alltrainonce/0000}{01}{15}
    % \end{minipage}
    % \begin{minipage}[t]{\galleryfigurewidth\linewidth}
    %     \animategraphics[width=\linewidth,autoplay=True]{30}{gifs/perturb/000}{072}{102}
    % \end{minipage}


    % \vspace{-15px}
    
    % \begin{subfigure}[t]{0.28\linewidth}
    %     \subcaption*{\tiny Cross-person motion. Left pose, right output.}
    % \end{subfigure} 
    % \begin{subfigure}[t]{0.28\linewidth}
    %     \subcaption*{\tiny Improved FE. Left 256px, right 512px.}
    % \end{subfigure} 
    
    % \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    %     \subcaption*{\tiny Ours.}
    % \end{subfigure} 
    % \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    %     \subcaption*{\tiny No pretrain.}
    % \end{subfigure}
    % \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    %     \subcaption*{\tiny All train at once.}
    % \end{subfigure}
    % \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    %     \subcaption*{}
    % \end{subfigure}
% \vspace{-10px}
\caption{
    Improved FE. Left 256px, right 512px.
    % For each image, left is pose, and right is output. 
    % The first two images in each subfigure are frames from the video. 
    Click the last image to play the embedded clips with Acrobat Reader.
    % \textit{\small Zoom in for detail. The first two images in each subfigure are frames from the video. Click the last images to play the embedded clips with Acrobat Reader.}
}
% \vspace{-15px}
\label{fig:512FE}
\end{figure}




==> figure/ablation_videolength.tex <==
\begin{figure}[htp]
\newcommand{\galleryfigurewidth}{0.24}
\centering
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Frame1}
\end{subfigure}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Frame2}
\end{subfigure}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Frame3}
\end{subfigure}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Frame4}
\end{subfigure}
    \begin{minipage}[t]{\linewidth}
    \centering
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_videolength/1/000116.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_videolength/1/000164.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_videolength/1/000208.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_videolength/1/000226.png}
        \end{minipage}
        \subcaption{Fine-tuning with one-minute videos}
    \end{minipage}

  \begin{minipage}[t]{\linewidth}
    \centering
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_videolength/5/000116.jpg}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_videolength/5/000164.jpg}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_videolength/5/000208.jpg}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_videolength/5/000226.jpg}
        \end{minipage}
        \subcaption{Fine-tuning with five-minute videos}
    \end{minipage}
    

\caption{
  Qualitative results with different video lengths for fine-tuning.
}
\label{fig:ablation.videolength}
\end{figure}


==> figure/audio_driven.tex <==

\begin{figure}[htp]
% \newcommand{\galleryfigurewidth}{0.092}
\newcommand{\galleryfigurewidth}{0.30}
% \newcommand{\galleryfigurewidthsrc}{0.14}
\centering
    %%%%
    \begin{minipage}[t]{\linewidth}
    \centering
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/audio_driven/crop_mxy.jpg}
            \includegraphics[width=\linewidth]{image/audio_driven/crop_oliver.jpg}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/audio_driven/mxy_pose_000096.jpg}
            \includegraphics[width=\linewidth]{image/audio_driven/oliver_pose_000242.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/audio_driven/mxy_000096.png}
            \includegraphics[width=\linewidth]{image/audio_driven/oiver_000242.png}
        \end{minipage}

    \end{minipage}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Appearance}
\end{subfigure}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Audio-driven pose}
\end{subfigure}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Output}
\end{subfigure}
\caption{
Examples of audio-driven results.
}
\label{fig:sup.audio_driven}
\end{figure}


==> figure/bad_pose.tex <==

\begin{figure}[htp]
% \newcommand{\galleryfigurewidth}{0.092}
\newcommand{\galleryfigurewidth}{0.30}
% \newcommand{\galleryfigurewidthsrc}{0.14}
\centering
    %%%%
    \begin{minipage}[t]{\linewidth}
    \centering
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badpose/badpose_lx_000073.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badpose/badpose_out_000073.png}
        \end{minipage}

    \end{minipage}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Bad pose}
\end{subfigure}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Bad output}
\end{subfigure}
\caption{
Bad case with the bad pose.
}
\label{fig:sup.badpose}
\end{figure}


==> figure/badcase.tex <==

\begin{figure}[htp]
% \newcommand{\galleryfigurewidth}{0.092}
\newcommand{\galleryfigurewidth}{0.30}
% \newcommand{\galleryfigurewidthsrc}{0.14}
\centering
    %%%%
    \begin{minipage}[t]{\linewidth}
    \centering
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badcase_largepose/ref.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badcase_largepose/hzy_badpose_000005.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badcase_largepose/out_000005.png}
        \end{minipage}
        \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
                    \subcaption*{Appearance}
        \end{subfigure}
        \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
            \subcaption*{Large pose variation}
        \end{subfigure}
        \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
            \subcaption*{Bad output}
        \end{subfigure}
        \subcaption{}
        \label{fig:sup.badcase.largepose}
    \end{minipage}
    \begin{minipage}[t]{\linewidth}
    \centering
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/ablation_face/lx_o/000001.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badpose/badpose_lx_000073.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badpose/badpose_out_000073.png}
        \end{minipage}
        \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
            \subcaption*{Appearance}
        \end{subfigure}
        \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
            \subcaption*{Inaccurate pose}
        \end{subfigure}
        \begin{subfigure}[t]{\galleryfigurewidth\linewidth}
            \subcaption*{Bad output}
        \end{subfigure}
        \subcaption{}
        \label{fig:sup.badcase.badpsoe}
    \end{minipage}
\caption{
Limitations. When the driven mesh is of large variation or inaccurate, the generated frame will be unsatisfactory.
}
\label{fig:sup.badcase}
\end{figure}


==> figure/facesgdm.tex <==
\begin{figure}
  \centering
   \includegraphics[width=1.0\linewidth]{image/faceDM.pdf}
   \caption{
   }
  \label{fig:facedm}
\end{figure}

==> figure/intro.tex <==

\begin{figure}[h]
  \centering
    \includegraphics[width=1.0\linewidth]{image/intro.png}
  \caption{
  }
  \label{fig:intro}
\end{figure}

==> figure/large_pose.tex <==

\begin{figure}[htp]
% \newcommand{\galleryfigurewidth}{0.092}
\newcommand{\galleryfigurewidth}{0.30}
% \newcommand{\galleryfigurewidthsrc}{0.14}
\centering
    %%%%
    \begin{minipage}[t]{\linewidth}
    \centering
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badcase_largepose/ref.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badcase_largepose/hzy_badpose_000005.png}
        \end{minipage}
        \begin{minipage}{\galleryfigurewidth\linewidth}
            \includegraphics[width=\linewidth]{image/badcase_largepose/out_000005.png}
        \end{minipage}

    \end{minipage}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Appearance}
\end{subfigure}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Large pose}
\end{subfigure}
\begin{subfigure}[t]{\galleryfigurewidth\linewidth}
    \subcaption*{Bad output}
\end{subfigure}
\caption{
Bad case with large pose.
}
\label{fig:sup.largepose}
\end{figure}


==> sec/2_related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\subsection{Talking Face Generation}
Talking face generation methods~\cite{prajwal2020wav2lip, zhang2023sadtalker, cheng2022videoretalking, wang2021facevid2vid} generate human videos with various expressions and poses conditioned on a given audio or motion, which can be categorized into two types: editing facial regions or generating dynamic head videos.
Editing-based techniques, such as Wav2Lip~\cite{prajwal2020wav2lip} or VideoRetalking~\cite{cheng2022videoretalking}, face the problem of lip-gesture inconsistency.
Usually, the gestures are fixed for different talking content.
Generating dynamic head video requires methods to create head videos conditioned on given audio or motion, where head motions are accomplished by different manners such as motion flow~\cite{yin2022styleheat}, 3D landmarks~\cite{wang2021facevid2vid, zhang2023sadtalker}, self-supervised training~\cite{pang2023dpe}, etc.
Although producing high-quality and highly realistic facial videos, talking face generation is limited by its interest area and cannot achieve full-body human video generation.
 
\subsection{Pose-guided Human Video Generation}
To generate human video with body and hand, pose-guided methods are the most popular approaches.
Early work focuses on the problem of motion transfer~\cite{motiontransfer_balakrishnan2018warpingbyICCV2021, motiontransfer_chan2019everybodydance, motiontransfer_siarohin2019fomm, motiontransfer_liu2019liquidwarpinggan, motiontransfer_siarohin2021mraa, motiontransfer_zhao2022tpsmotion, motiontransfer_siarohin2023unsupervised, motiontransfer_wang2022lia, motiontransfer_yang2022delving} methods.
Balakrishnan et al.~\cite{motiontransfer_balakrishnan2018warpingbyICCV2021} separate a scene and transform each part to synthesize.
% Chan et al.~\cite{motiontransfer_chan2019everybodydance} utilize pretrained pose to represent the body and transfer the appearance of the identity in the training dataset.
% Liu et al.~\cite{motiontransfer_liu2019liquidwarpinggan} decouple the task into mesh recovery, flow composition, and warping.
FOMM~\cite{motiontransfer_siarohin2019fomm} and MRAA~\cite{motiontransfer_siarohin2021mraa} propose unsupervised body representation and warping to transfer, while LIA~\cite{motiontransfer_wang2022lia} employs latent space.
TPS~\cite{motiontransfer_zhao2022tpsmotion} introduces thin plate spline transformation into a motion transfer task, and UVA~\cite{motiontransfer_siarohin2023unsupervised} presents a differential volumetric representation.
Besides the coarse-grained motion transfer setting, researchers~\cite{cogesture_ginosar2019learningstylegesture, cogesture_qian2021speechdrivetemplates, cogesture_zhou2022audiodriven-videomotiongraphs, cogesture_liao2020speech2video} apply these kinds of methods into human video generation with face, body, and hand.
However, constrained to the capability of these models, these methods potentially generate human videos with apparent artifacts.

With the progress of diffusion models~\cite{ho2020ddpm, rombach2022ldm}, some works introduce them into pose-guided human video generation.
Follow-your-pose~\cite{ma2023followyourpose} introduces a two-stage training to get a pose-guided video diffusion model.
DreamPose~\cite{karras2023dreampose} proposes a vision and pose controlled diffusion on fashion dataset to animate a body image.
DisCo~\cite{wang2023disco} focuses on human dance generation, utilizes multiple ControlNet on pose and background, and introduces a pretraining strategy to improve generalizability.
Nonetheless, these methods concentrate on coarse-grained body video generation, which is limited to the poor quality of face and hands. 
Besides, due to the randomness of the diffusion model, these methods struggle with temporal consistency.
The proposed system, by proposing a simple yet efficient multi-frame inference strategy, could improve the temporal consistency of image-based diffusion models.
%\ziyao{MagicAvatar~\cite{zhang2023magicavatar} is the most relevant work with ours, which supports avatar animation from multiple motion inputs (e.g., human pose, depth, DensePose), however, it is still unsubstantiated of the ability to generate talking lips.}

\subsection{Video Diffusion Models}
Due to the powerful capabilities of diffusion models, researchers in recent years have started to explore their potential in video generation, and much progress has been made in video generation~\cite{ho2022imagenvideo, singer2022makeavideo, blattmann2023alignyourlatents, chen2023videocrafter1, ge2023preserveyourcorrelation} and video editing~\cite{chai2023stablevideo, QI_2023fatezero, yang2023rerender}.
GEN-1~\cite{esser2023gen1} extends the image diffusion model with a temporal module and utilizes depth to control the structure.
Tune-A-Video~\cite{Wu_2023_tuneavideo} fine-tunes 3D U-Net in image diffusion model on a one-shot video to learn the motion and then edits the video content with text prompts.
AnimateDiff~\cite{guo2023animatediff} trains a temporal module with a fixed image diffusion model and can be applied to personalized weights.
% controlvideo, animatediff
While VDMs possess strong video generation capabilities, the ability to control human motion and maintain appearance needs further improvement.
In contrast, we tune the foundation diffusion model to learn the mapping from motion to a specific anchor appearance in a ``binding'' fashion following a pretrain-finetuning paradigm.
%and VDMs cannot be directly used for synthesizing human videos.\ziyao{not exactly}

%\subsection{Human Nerf}

==> sec/bak/1_intro_bak.tex <==
\section{Introduction}
\label{sec:intro}

2D human video generation is an essential task, which aims at generating human video with expression, torso and gesture with the input audio, text or motion condition.
This task has widely applications in education, entertainment, online conferencing, VR and etc. 
% 理想的2D虚拟人视频应该像真实的人类视频一样，在具有逼真的外观的前提下，能够做出自然的嘴型、手势和全身动作。
The ideal generated human video should resemble real human videos, with a realistic appearance, while being able to produce natural facial movements, gestures, and full-body actions.

% 为了生成2d人类视频，基于深度生成模型的方案是现在的主流方案。
Past works have explored GAN-based approaches. However, the efficacy of GAN-based approaches is more pronounced specifically on the talking face generation~\cite{prajwal2020wav2lip, wang2021facevid2vid, zhang2023sadtalker, pang2023dpe}, where only the facial region have been edited.
When expanding beyond facial region generation, current GAN-based methods like motion transfer~\cite{motiontransfer_zhao2022tpsmotion, motiontransfer_siarohin2021mraa, motiontransfer_siarohin2019fomm} and co-speech generation~\cite{cogesture_qian2021speechdrivetemplates, cogesture_zhou2022audiodriven-videomotiongraphs} can generate other body parts such as the torso and hands, while the resulting quality is not entirely satisfactory.
This is primarily attributed to the inherent difficulty of current GAN models to generate human bodies with complex motions.
Diffusion models~\cite{ho2020ddpm} have been proven to achieve promising generation quality on human image generation~\cite{rombach2022ldm}. Compositing with pose or depth condition~\cite{zhang2023controlnet}, current text-to-image diffusion models, such as Stable Diffusion~\cite{rombach2022ldm}, can synthesize human body with specific gesture, pose and expression, and can keep identity by personalized fine-tuning methods~\cite{ruiz2023dreambooth, gal2022TI, kumari2023customdiffusion, hu2021lora}.
However, due to the randomness of the diffusion process, image diffusion models cannot be directly applied to generate temporal human video.
Existing video diffusion models~\cite{ho2022imagenvideo, singer2022makeavideo}, which are proven to generate temporal-consistent videos with simple motion and nature scenes, have been investigated to produce human video generation.
DreamPose~\cite{karras2023dreampose} modifies Stable Diffusion to be controlled by input image and pose, and animates a still human image conditioned on given fashion motion.
DisCo~\cite{wang2023disco}, which also supports image input, applies pose and background ControlNet~\cite{zhang2023controlnet} to composite different motion and scenes with a pretraining strategy, and achieves promising human dance generation results on generalization.
However, existing diffusion-based approaches are still difficult to synthesize facial details, exact gestures, and temporal frames, which is not sufficient for human video generation.


% 方法部分
% 方法框架：单人物微调+3d mesh映射到人类视频。方法框架这一段论证一下这么设计的合理性，说现有落地方案都这么做的
% 具体实现：1、2、3
In this paper, to achieve 2D human video generation, we formulate this task as training on a specific identity and appearance with less than 5 minutes video, and mapping animatable 3D mesh motion sequence to human video.
We have noticed that there are already existing technological solutions capable of generating corresponding 3D human mesh with lip, gesture and body motion conditioned on either audio~\cite{yi2023talkshow}, text inputs~\cite{} or just motion capture. 
By integrating these existing multi-modality driven solutions, our task formulation can align with established human video generation implementations, such as HeyGen~\footnote{https://www.heygen.com/}, ZenVideo~\footnote{https://zenvideo.qq.com/}, and D-ID~\footnote{https://www.d-id.com/}, which are accomplished by talking face generation and cannot achieve ideal human video generation.
\input{figure/intro}
% 现有的2D数字人技术关注于头部的生成。例如，一些app如heygen、腾讯智影数字人、剪映数字人等软件可以生成指定ip的说话视频，上传一段5分钟左右特定ip的视频，就能得到模型就能够生成2D数字人视频。现有方法虽能进行高质量talking生成，但是视频的姿态动作往往是固定的、预先拍摄的，不能生成动作视频
% Existing 2D digital human technology focuses on generating the head. For example, some apps such as HeyGen~\footnote{https://www.heygen.com/}, ZenVideo~\footnote{https://zenvideo.qq.com/}, and D-ID~\footnote{https://www.d-id.com/} can create speaking videos of specified or unspecified person. By uploading a  video, the model can generate 2D digital human videos with speaking and gesture. While current methods are capable of producing high-quality human video, the video's poses and actions are often fixed and pre-recorded, and they cannot generate action videos.
% This is because existing methods primarily concentrate on generating the "talking face," allowing for edits to facial expressions and poses. However, constrained manipulated/interested region of talking face generation limits the real-world application scenarios, and lacks the capability to address the lip-gesture inconsistency issue. This approach cannot produce the desired digital human video.

% Apart from the solutions focused on generating the talking face, there is also a portion of work dedicated to creating motion videos for the human body trunk. Existing technology solutions capable of producing realistic 2D videos include motion transfer, video generation, and human NerF.
% Motion transfer methods focus on coarse-grained body movements and cannot generate precise mouth shapes and hand motions, leading to suboptimal video quality (TPS, NIPES2022\_ANGIE, dreampose, disco).
% General video generation methods struggle to consistently generate character identities and do not support the generation of complex movements.
% While NERF human can produce high-quality human body reconstructions, it often requires the collection of targeted multi-view video data. Additionally, driving existing NERF human models to generate 2D videos presents a challenge.
% While these approaches are capable of generating human body videos, their video quality or data collection can be challenging, and these methods have not yet focused on crucial detailed regions such as the face and hands, making them insufficient for generating the ideal 2D virtual humans.

% 为了生成理想的human video，我们提出了一套uniform的生成框架。在这个框架中，我们使用语音、文本或者动作来得到驱动视频中人体的表情、手势和躯干动作，然后再从动作序列渲染出人体视频。现在已经开展了前一部分的研究，如co-speech gesture generation，因此我们本工作的重点放在后面这个阶段：如何从细粒度的人体动作序列生成出真实的human video。
% To generate the ideal human video, we propose a unified generation framework. In this framework, multi-modality information such as speech, text, or actions is utilized to drive the expressions, gestures, and body movements of the human in the generated video. Substantial research has already been conducted on the first part, such as co-speech gesture generation. Therefore, the primary focus of our work is on the latter stage: how to render authentic human videos from fine-grained human motion sequences.
% \ziyao{add the difficulty to achieve this goal}

We propose a novel diffusion-based framework to accomplish the above formulation.
\textbf{Appearance and Identity Control}: We utilize a pre-training followed by specific person fine-tuning approach.
To control the appearance, we replace the text clip input with image clip on pretrained Stable Diffusion~\cite{rombach2022ldm}, and training on over 30 hours of human body videos.
After finishing pre-training, we fine-tune the appearance model with 3-5 minutes of data for the desired person, resulting in a stable appearance model.
\textbf{Structure-Aware Body Generation}: Despite coarse body landmarks~\cite{} or denspose visualization~\cite{}, we use the human body mesh rendered by SMPL-X~\cite{pavlakos2019smplx} as the motion sequence to provide accurate structure information, and employ a ControlNet~\cite{zhang2023controlnet} combined with a pretrained diffusion models to learn the corresponding mapping from actions to human body images.
\ziyao{Besides, we propose a hand-weighted inference strategy to improve the generation quality of hands.}
\textbf{Identity-Specific Face Enhancement}: Face generation results occupies an essential part of identity perception and human video quality. We propose a face enhancement module by revising the face part of the body generation video.
We apply an identity-specific face inpainting network with a head mesh ControlNet to rerender a better face results.
\textbf{Sliding Window Temporal Strategy}:
The key importance of human video is the temporal consistency and the capability to generate arbitrary long video.
Based on above researches, we employ training-free all-frame cross-attention modulate to improve continuity between frames, and we propose a sliding window smoothing strategy on diffusion output noise to extend the limitation to generate long video.
% \textbf{Super-Resolution}: We have developed a specific person super-resolution model based on DreamBooth. When combined with video editing methods, it can easily enhance the generated videos to high-quality 1024px resolution.
All of these operations can be performed within a practical time cost on a single 40G A100 GPU.

% 总结
% 我们提出了一套可行的方案可以生成高质量、多层次动作的human video，并且能够控制住视频内的外观和id。我们提出的框架结合设计的方法打通了数字人生成的通路，并可以启发后续这一系列2D数字人的研究和实用。我们的方法可以结合现有的人体动作序列生成方法并得到很好的效果，在本文中我们结合现有的audio2mesh的方法并能得到很惊艳的效果。我们跟talking face、motion transfer、pose-guided video generation和human nerf的方法都进行了比较，定性和定量实验都证明了我们提出方法框架的有效性。
We propose a practical solution for generating high-quality, multi-layered human videos with the ability to control motions including lip, expression, gesture and body action. 
The framework we have presented, along with the designed methods, opens up pathways for digital human generation and can inspire further research and practical applications in the realm of 2D digital humans. 
Our approach can be effectively combined with existing human motion sequence generation methods, and in this paper, we have showcased remarkable results by integrating it with the existing Audio2Mesh method.
We take experiments on \ziyao{10} different identities and appearances, and we conduct qualitative and quantitative results, comparing our approach with methods such as talking face, motion transfer, pose-guided video generation. The results from these experiments validate the effectiveness of our proposed method framework.
% Past human video generation methods focus on talking face generation~\cite{} and motion transfer~\cite{}. Talking face generation edits the expression and pose of the input face by given speech or motion. Despite the progress in this field, constrained manipulated/interested region of talking face generation limits the real-world application scenarios, and lacks the capability to address the lip-gesture inconsistency issue.
% speech-driven and motion-driven是不一样的，我们实际上是speech-driven，虽然现在没加相关特征。
% In recent years, co-speech gesture generation~\cite{} has raised interests in research community, where 



==> sec/bak/3_method_back.tex <==
\section{System Overview}

% Stable Diffusion~\cite{rombach2022ldm} is a text-to-image latent diffusion model which consists of a VAE, UNet, and a text-encoder.

% \paragraph{SMPL-X}


%\subsection{System Overview}
\label{sec:method.overview}
% 对于我们任务中使用的pose，我们的方法输入一个由smpl-x渲染出来的3d mesh序列，并将其渲染成特定人物的视频。
% 在输入输出上，我们跟之前已有方法的主要不同是，输入上我们使用的是smpl-x渲染的人体3d mesh，之前的方法要么使用pose landmarks，要么使用denspose，其问题在于对精细部位（脸部和手）描述不足，同时视频上不够连续，这导致了之前方法在一些关键部位的生成上存在问题，且达不到想要刻画的部位。
% 在输出上我们在instance-level的视频上进行训练，对于
\paragraph{Setting.}
Although existing approaches~\cite{wang2023disco, karras2023dreampose} mostly frame human video generation as generating video from a single or few-show appearance image, such formulation made this task into an ill-posed problem. 
we believe that it is practical to formulate this task as learning from a video of one identity.
% In this formulation, achieving consistency in identity and appearance across video frames becomes challenging, because models need to ``guess'' what appearance is with unseen pose. 
% Moreover, when considering accurately reflect the identity of a real person in a video, this setup is not reasonable. 
In real-world digital anchor applications, such as ZenVideo \ziyao{virtual anchor}, users seeking to customize a character are often required to upload a brief video capturing the desired pose and movements, and our task formulation aligns with these existing practical scenarios.
Regarding the difficulty of data collection, aside from user-generated videos, situations where capturing is impractical, such as for deceased actors or reaging an actor's appearance, permit the use of artificially composed training data through manual cropping of existing materials. In the experimental chapter, we will demonstrate the synthetic effects achieved through two manners:0 green screen capturing and manual cropping of network videos for specific identity synthesis. 
\paragraph{Workflow.}
The whole pipeline of our system, ``Make-Your-Anchor'', is displayed in Fig.~\ref{fig:pipeline}.
Our system comprises two primary components: Frame-wise Motion-to-Appearance Diffusing to training a new frame-level identity model, and Batch-overlapped Temporal Denoising to inference in video-level.
In Frame-wise Motion-to-Appearance Diffusion, an image diffusion model $\hat{X}_\theta$ with appearance and pose control are trained by anchor video frames $F^{t} = \{f_i^t, f_2^t, ..., f_n^t\}$ and corresponding 3D mesh sequences $P^t=\{p_1^t, p_2^t, ..., p_n^t\}$.
A face enhancement module $\hat{X}_\theta^f$ is further optimized to improve the face quality.
We train our models with two-stage training strategy, where we firstly pretrain our diffusion model with multi-id dataset, and then fine-tune on a new identity to accomplish training.
In Batch-overlapped Temporal Denoising, we extent the frame-level model $\hat{X}_\theta$ into video-level model $\hat{X}_\theta^V$, and the inference poses $P=\{p_1, p_2, ..., p_n\}$ are feed into our model to generate video. To overcome the length limitation of $\hat{X}_\theta^V$, the overlapped temporal denoising algorithm is proposed to produce arbitrary long video.


\paragraph{Input.}
Based on the above setting, ours system requires an anchor-style video of one identity for training and input pose sequences for inference, and the final output is human motion video frames $F=\{f_i, f_2, ..., f_n\}$ with temporal appearance.
The given video for training contains lip, body, gesture movements in sitting or standing, and the video length is at least 1 minutes and not exceeds 5 minutes. 
\ziyao{
This training setting is similar with preceding co-speech work~\cite{cogesture_zhou2022audiodriven-videomotiongraphs}.
}
% and we concentrate on generating specific human motion videos based on a given video not exceeding 5 minutes.
% Our method primary concentrate on the motion and appearance quality of the output video.
We utilize human 3D mesh rendered from SMPL-X parameters~\cite{pavlakos2019smplx} as our input pose sequence $P=\{p_1, p_2, ..., p_n\}$.
% Current methods applied human pose~\cite{cao2017openpose} or DensePose~\cite{guler2018densepose}, which are coarse representation of human body.
We believe that the smoothness and accuracy of input pose condition influences the temporal consistency of output video, and the 3D human mesh already contains sufficient structural information about the motion to generate smooth video, especially in hand gesture.
Besides, a reference image $I_r$ is used as our appearance input for our model\ziyao{, which primarily works on pre-training stage}.
% \ziyao{}
% pose和appearance输入网络，得到一开始的body结果，然后我们对
% We designed Structure-Guided Diffusion Model to accomplish body generation with pose and appearance input.
% We introduce a two-stage training strategy to train our model, where pre-training on multi-identity data to obtain fundamental ability and then fine-tuning on one instance video to generate stable anchor results.
% To further improve the quality of appearance and motion, we propose identity-specific face enhancement to revise the essential face region, and sliding window temporal strategy to overcome the limitation of video diffusion models to generate long temporal video.




% \paragraph{Formulation}
% % hvg的基础设定为，给定一段动作序列和分身外观信息，生成其动作视频。
% % 虽然现有方法大多设定为通过一张图片推断出该人物的其他动作，但这样使得任务变成了一个欠定问题，如果想要真实的反映出一个实际存在的人物id的话，这样的设定并不合理，而且难以达到视频时序上身份和外观一致的目标。特别上有一定角度变化的情况下，如手部复杂的运动，现有基于warpping的方法大多难以准确的对不同姿态下的手部进行建模于与生成。
% % 考虑以上的这些问题，并结合实际可以接受的代价，我们将hvg任务设定为在给定一小段不超过5分钟长度的视频的情况下，根据一段动作序列来生成他的动作视频。
% % 在一些实际应用中，如zenvideo数字人，当用户想要定制一个人物的数字人，其会要求用户上传一段几分钟的视频，将视频中的姿态动作作为视频模板进行使用，因此我们的设定跟已有的实际应用场景是一致的。
% % 从数据收集的难易度上看，除开用户自己拍摄的视频外，在不方便进行拍摄的情况下，如已经故去的演员，或者想要年轻化的演员视频时，通过人工裁剪已有素材组合成训练数据也是一个可接受可用的设定。在实验章节我们会展示通过绿幕拍摄和人工裁剪网络片段两种方式获得的特定id的合成效果。
% The basic formulation of human video generation is that given pose sequence $P=\{p_1, p_2, ..., p_n\}$ and identity information $I$, generative models produce human motion video frames $F=\{f_i, f_2, ..., f_n\}$ with temporal appearance.

% Particularly, in cases with significant angular variations, such as complex hand movements, many existing warping-based methods~\cite{motiontransfer_zhao2022tpsmotion, cogesture_qian2021speechdrivetemplates} struggle to precisely generate hands under different poses.

% Taking into consideration the aforementioned issues and practical acceptability, we define the human video generation task as generating specific human motion videos based on a given video not exceeding 5 minutes.
% In real-world human video generation applications, such as ZenVideo, users seeking to customize a character are often required to upload a brief video capturing the desired pose and movements. Therefore, our task formulation aligns with existing practical scenarios.
% Regarding the difficulty of data collection, aside from user-generated videos, situations where capturing is impractical, such as for deceased actors or reaging an actor's appearance, permit the use of artificially composed training data through manual cropping of existing materials. In the experimental chapter, we will demonstrate the synthetic effects achieved through two methods: green screen capturing and manual cropping of network videos for specific identity synthesis. 


\section{Method}

% 我们的方法的目标是根据给定的动作序列能够生成连续的人类视频。
% 为此，我们的方法基于sd1.5进行修改，并且我们根据以下几个关心的主要问题进行设计：身份和外观保持，动作生成，以及视频一致性。为此，提出了我们的几个模块：1. 2. 3. 4.
Our method aims to produce human video conditioned on given pose sequence.
% To accomplish this, our method is based on pretrained latent diffusion model~\cite{rombach2022ldm}, Stable Diffusion v1.5, and adapt it according to our primary concerns: identity and appearance control, structure-aware pose generation and temporal consistency.
% The overview of our method will be displayed in Section~\ref{sec:method.overview}.
We introduce our network architecture and training strategy in Section~\ref{sec:method.arch} to accomplish image-level appearance and body structure control.
In Section~\ref{sec:method.slindingwindow}, batch-overlapped temporal denoising is proposed to generate arbitrary long cross-frame consistent video.
% Combined with our proposed strategies in Section~\ref{sec:method.strategy}, including two-stage training, Identity-Specific Face Enhancement and Sling Window Temporal Strategy, our method achieves realistic and temporal human video generation.

\input{figure/pipeline}

\paragraph{Preliminaries.}
Diffusion Models~\cite{ho2020ddpm} are generative models to learn a diffusion process that generates the probability distribution.
Given an initial noise $\epsilon \sim \mathcal N(0, 1)$ and a condition $c$, the trianing loss of diffusion models can be written as:
\begin{equation}
    \mathbb{E}_{x,c,\epsilon,t} [w_t || \hat{X}_{\theta} (\alpha_t x + \sigma_t \epsilon, t, c) -\sigma ||^2_2 ],
\end{equation}
where $\hat{X}_{\theta}$ is the diffusion model, $x$ is the ground-truth image, $\alpha_t$, $\sigma_t$, $w_t$ are hyperparameters, and $t$ is the diffusion timestep.
To generate an image, the final image $x_0$ is denoised from an initial noise $x_T$ with multiple steps.
For example, DDPM~\cite{ho2020ddpm} sampling is:
\begin{equation}
    x^{t-1} = \frac{1}{\sqrt{\alpha_t}} (x^t - \frac{1-\alpha_t}{\sqrt{1-\overline{\alpha}_t}} \hat{X}_{\theta} (x^t, t, c) )  + \sigma_t \epsilon,
\end{equation}
where $x^{t-1}$ is denoised from $x^t$ by the output of diffusion model $\hat{X}_{\theta}$ at timestep $t$.


\subsection{Frame-wise Motion-to-Appearance Diffusing}
\label{sec:method.arch}
\paragraph{Structure-Guided Diffusion Model.}
We propose Structure-Guided Diffusion Model (SGDM), modified from pretrained text-to-image Stable Diffusion V1.5~\cite{rombach2022ldm}, to achieve appearance and motion control.
 The model architecture is shown in Fig.~\ref{fig:pipeline}.
% \paragraph{Appearance Control}
% \label{sec:method.appnet}
% We utilize a pre-training followed by specific person fine-tuning approach.
To control the appearance, we replace the text CLIP~\cite{radford2021clip} input $C_{T} \in R\times d$ with image CLIP feature $C_{I} \in hw\times d$ to the cross-attention module:
\begin{equation}
    C_{I} = CLIP_{Image}(I_r),
\end{equation}
where the appearance feature is extracted by image CLIP from reference image $I_r$, and then feed into Stable Diffusion's U-Net.
We utilize the CLIP feature map before global pooling layer which provides more fine-grained appearance information ~\cite{wang2023disco}.
% , and training on over 30 hours of human body videos.
% After finishing pre-training, we fine-tune the appearance model with 3-5 minutes of data for the desired person, resulting in a stable appearance model.
% \paragraph{Structure-Aware Body Generation}
% \paragraph{Structure ControlNet}
% \label{sec:method.controlnet}
To embed the 3D mesh condition into the generation process, we employ a ControlNet~\cite{zhang2023controlnet} module to learn the corresponding mapping from pose $P$ to human body images.
ControlNet have been proven to condition generation based on pose, depth, canny, etc.
It adds an extra condition branch to Stable Diffusion's U-Net by copying U-Net's encoder and adding a zero-convolution layer between the input condition image and encoder, then the encoder's layer-wise feature maps are added on the U-Net's up layers:
\begin{equation}
    F_{up} = F_{up} + W_c \times ControlN(P),
\end{equation}
where $F_{up}$ is the feature map of U-Net's up layers, $ControlN$ is the ControlNet branch, $P$ is the input 3d mesh and $W_c$ is a hyperparameter to weight the control condition.
We found it is sufficient to control motion by training a ControlNet from scratch.
The generation of human image can be abbreviated as:
\begin{equation}
    x^0 = \hat{X}_\theta(P, C_{I}, x^T)
\end{equation}
where $x^T$ is the input latent.
% \ziyao{need a diffusion equation}
% \begin{equation}
%     Output = DM(I_r, P).
% \end{equation}
%\ziyao{
%And a large $W_c$ would bring a more condition-weighted output, which benefits the hand gesture generation. 
%Besides, we propose a hand-weighted inference strategy to further improve the generation quality of hands.
%}

\paragraph{Identity-Specific Face Enhancement.}
\label{sec:method.faceenhance}
% 我们注意到，整图生成的脸部区域往往难以获得满意的质量，我们认为这是因为脸部区域在整图上较小，在整图mse loss的情况下模型难以关注到脸部这么小的区域。为此，我们选择了一种inpainting style的方式对已生成的脸部区域进行revision。
We observe that it is challenging to generate satisfied face from a holistic human generation.
From our perspective, this phenomenon arises due to the relatively diminutive size of the facial region within the entire image. 
With the training loss on holistic human image, the model encounters difficulty in fitting the small facial area.
To address this, we opted for an inpainting-style approach to revise the facial region from the holistic generated body.
In detail, we adapt the SGDM with face inpainting to Face SGDM, as shown in Fig.~\ref{fig:facedm}.
The ready-to-revise face is cropped from the body generation, and the inpainting region is segmented via a facial mask $M$. We replace the input for SGDM' U-Net with a concatenation of facial mask, masked face $x_M$ and the original input latent. The input appearance and motion condition is aligned with corresponding reference and 3D mesh image. The generation process can be abbreviated as:
\begin{equation}
    x_f^{0} = \hat{X}_\theta^f(P^f, C_{I}^f, x_f^{T}, M, x_{M}),
\end{equation}
where $\hat{X}_\theta^f$ is the Face SGDM, $x_f^{0}$ is output, and $x_f^{T}$ is input latent.
The inpainting style face enhancement prevents the requirements of paired data, and train on only real data.

% inpainting的好处：直接在真实图像上训练，不需要pair data

\paragraph{Two-Stage Training Strategy.}
\label{sec:method.twostagetrain}
% 对于上述能够实现外观和动作控制的模型框架，我们提出了一个两阶段的训练策略来训练我们的网络。具体而言，我们先使用多id的数据对模型进行预训练，然后再在arbitraty id上用一段视频进行微调。在多id上进行预训练可以帮助模型学到如何控制生成的motion，同时多id外观训练能提高模型对单id微调的泛化性；而单id的微调可以帮助模型固定我们想要的实际人物的外观信息，从而获得一个稳定的外观输出。
% 具体而言，对于预训练阶段，为了排除外观对人体信息学习的干扰，我们将target图片的前景人体进行了抠离，同时image clip可以帮助模型对不同id的认识，帮助对外观的泛化。
% 在单id微调阶段，我们选择背景和前景一起进行训练。这样模型在能够快速泛化到新人物id的前提下，也能够记住背景，从而生成和谐的anchor视频。跟disco不同的是，我们没有选择将前背景分开解耦的方式，因为背景可以通过绿幕抠图的方式进行替换。

We propose a two-stage training strategy to train our network. 
We first pretrain the model using multiple identities data, and then fine-tune it on one video of an arbitrary identity. Pre-training on multiple identities helps the model learn how to control motion, and enhances generalization for fine-tuning on a new identity. Fine-tuning on a new identity helps the model capture the desired appearance information precisely of the specific individual, resulting in a stable appearance output.

Specifically, to eliminate the interference of background on learning human information in pre-training stage, we segment the foreground human body from the target images. 
% \ziyao{discuss the necessary of image clip}
During the fine-tuning stage on a single identity, we chose to train both the background and foreground together. This approach allows the model to quickly generalize to new individual identities while also remembering the background, thereby generating harmonious anchor videos. 
\ziyao{Unlike Disco~\cite{wang2023disco}, we do not choose to decouple the foreground and background because the background can be replaced through green screen segmentation.}

% \subsection{Sliding Window Temporal Strategy}
\subsection{Batch-overlapped Temporal Denoising}
\label{sec:method.slindingwindow}
% 在图像级别训练，视频级别推理，同时使用overlap window来做长视频生成。这里需要多写一点公式，需要VDM的表达。
% 为了提升效果，我们在推理阶段将模型扩展为一个VDM，具体实现如下：
% 写一下attention的公式
% 同时，为了生成长视频，我们用了一个overlap slidng window smoothing的策略，从而生成长视频
% 写个算法更容易理解
% 我们以上的方法因为对于motion和appearance的控制，已经能够生成视频。但因为diffusion模型输出的随机性，帧之间依然存在不连续的现象。
% 之前一些工作已经验证了将图像dm的self attention扩展为帧间attention能够提升生成视频的一致性，因此我们的方法也将2d unet扩展为了3d unet，主要是
Our method mentioned above have been successful in generating human images by controlling both pose and appearance. However, due to the inherent randomness in the output of the diffusion model, there still exists discontinuity between frames.
Previous studies~\cite{khachatryan2023text2video, zhang2023controlvideo} have already demonstrated that extending self-attention in image diffusion model to cross-frame attention enhances the consistency of generated videos. 
Our approach involves extending the 2D U-Net to a 3D U-Net to get a training-free video diffusion model $\hat{X}_\theta^V$. Specifically, we utilize an all-frame cross attention module to replace the self-attention, which can be written as:
\begin{equation}
    Attention(Q, K, V) = Softmax(\frac{Q K^T}{\sqrt{d}})\cdot V,
\end{equation}
where $X^t=\{x_1^t, x_2^t, ... x_t^N\}$ is the input latent frames on diffusion timestep $t$ and $Q = W_Q \cdot X_t$, $K=W_K \cdot X_t$, $V=W_V \cdot X_t$ are attention weights. 

Another pivotal consideration is the limited generation length of video diffusion model, especially for the arbitrary length of an anchor video.
We propose an overlapped temporal denoising algorithm to extend the generation length which is illustrated in Algorithm~\ref{algorithm:temporal} and Fig.\ref{fig:pipeline}.
% 我们通过滑窗的方式，将一段长视频分成多个存在overlap的窗口。在所有窗口都经过vdm推理之后，我们对重叠的部分进行归一化，这样能保证结果正确。我们发现这样的方法就能简单有效地扩展vdm去生成任意长的视频。
We partition a long video input into multiple overlapped windows.
In each denoising step, the windows are feed one-by-one into our video diffusion model. 
Once all windows are handled, we normalize the overlapped noises between windows to ensure coherence, and then the all video frames are denoised by the smoothing noises.
After all denoising steps are executed, the final results present a long temporal video.
We observe that this simple approach effectively extends video diffusion model to generate videos of arbitrary length while keeps temporal consistency.

\input{algorithm/temporal}

\input{figure/facesgdm}


==> table/512FE.tex <==
\begin{table}
  \centering
  \resizebox{.8\linewidth}{!}{
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    Method                            & FID  &   FVD↓           &    LMD (Face)↓                    \\
    \midrule
    Ours                              & 40.33     &   139.82        &    1.44                   \\
    % Q5 w SMPL perturbation                 &   136.21        &    1.40               &  5.25                 \\
    % Q2 \& Q8 Cross-person motion                   &  145.33        &    1.69          &  5.66                \\
    FE w 512px                        & 39.73     &  140.18        &    1.35                              \\
    % Q11.1 Only train fine-tuning video          &  278.73        &    4.38           &   7.25                \\
    % Q11.2 All train at once                    &  178.79        &    1.56         &   6.01                \\
    % Metrics                              &    Ours   & Q2 \& Q8  & Q5      & Q6     &  Q11.1  & Q11.2 \\
    % \midrule
    %  FVD↓                                &    139.82 & 145.33    & 136.21  & 140.18 &  278.73 & 178.79 \\
    %  LMD (Face)↓                         &    1.44   & 1.69      & 1.40    & 1.35   &  4.38   & 1.56 \\
    %  LMD (Body)↓                         &    4.88   & 4.98      & 4.65    & —     &  5.34   & 4.77 \\
    %  LMD (Hand)↓                         &    5.41   & 5.66      & 5.25    & —      &  7.25   & 6.01 \\
    \bottomrule
  \end{tabular}
  }
  \vspace{-10px}
  \small
  \caption{ Numerical results of FE with 512px.}
  \label{tab:512FE}
  \vspace{-10px}
\end{table}


==> table/ablation_timecost.tex <==
\begin{table}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{@{}lccccccc@{}}
    \toprule
    Method                              & Pose2Img              &  TPS       & DreamPose           &    DisCo    & Ours   & Ours w/o TD    & 300 frames w/o TD          \\
    \midrule
    % \multicolumn{7}{l}{Same-domain Motion} \\
    % \midrule
    % Time cost                          &  77s            &  42s           & 610s         &    234s         & 407s         &  301s           & OOM        \\
    Time cost                          &  77s            &  42s           & 310s         &    154s         & 407s         &  301s           & OOM        \\
    Method type                        &  non-diffusion  &  non-diffusion & diffusion    &    diffusion    & diffusion    &  diffusion      & diffusion        \\
    Resolution                         & 640px           &  384px         & 512px        &    256px        & 512px        &  512px          & 512px      \\
    % \midrule
    % \multicolumn{7}{l}{Cross-domain Motion} \\
    % \midrule
    %  w/o TD                             &       48.84       &  18.20          &  344.85        &   1.45            &  4.74         &  5.61              \\
    % w/o FE                              &       40.84       &  16.18          &  124.10        &   1.56           &  -            &   -                \\
    \bottomrule
  \end{tabular}
  }
  % \vspace{-10px}
  \caption{Comparison of time cost to generate 300 frames. }
  \label{tab:ablation.timecost}
  % \vspace{-24px}
\end{table}


==> table/ablation_videotime.tex <==

\begin{table}[!ht]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{@{}lcccccc@{}}
    \toprule
    Fine-tuning with          & FID↓              & FVD↓           &    LMD (Face)↓    & LMD (Body)↓   & LMD (Hand)↓               \\
    \midrule
    One-minute videos         &  40.33            & 139.82         &    1.44           & 4.88          &  5.41    \\
    Five-minute videos        &  38.94            & 134.55         &    1.29           & 4.42          &  4.95     \\
    \bottomrule
  \end{tabular}
  }
  \caption{Ablation analysis of video length used for fine-tuning.}
  \label{tab:ablation_videotime}
\end{table}


% back
% \begin{table}[!ht]
%   \centering
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{@{}lcccccc@{}}
%     \toprule
%     Fine-tuning with                              & FID↓              &  FID-VID↓       & FVD↓           &    LMD (Face)↓    & LMD (Body)↓   & LMD (Hand)↓               \\
%     \midrule
%     One-minute videos         &  40.33            &  15.95          & 139.82         &    1.44           & 4.88          &  5.41    \\
%     Five-minute videos        &  38.94            &  15.45          & 134.55         &    1.29           & 4.42          &  4.95     \\
%     \bottomrule
%   \end{tabular}
%   }
%   \caption{Ablation analysis of video length used for fine-tuning.}
%   \label{tab:ablation_videotime}
% \end{table}


==> table/userstudy.tex <==
\begin{table}[!h]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{@{}lcccc@{}}
    \toprule
    \multirow{2}{*}{Method}                                               & Appearance        & Temporal      & Structure             & Overall           \\
                                                                          &  Preservation     & Consistency   & Preservation          & Quality           \\
    \midrule
    Pose2Img~\cite{cogesture_qian2021speechdrivetemplates}                & 3.36              & 2.38          & 1.59                  & 2.01              \\
    TPS~\cite{motiontransfer_zhao2022tpsmotion}                           & 2.03              & 2.10          & 1.18                  & 1.37              \\
    DreamPose~\cite{karras2023dreampose}                                  & 2.78              & 1.94          & 2.27                  & 1.94              \\
    DisCo~\cite{wang2023disco}                                            & 2.29              & 2.32          & 1.45                  & 1.72              \\
    Ours                                                                  & \textbf{4.23}     & \textbf{3.85} & \textbf{3.91}         & \textbf{4.03}     \\
    \bottomrule
  \end{tabular}}
  \caption{User study scores. The rating score is on a scale from one to five, where five is the highest score, and one is the lowest.}
  \label{tab:userstudy}
\end{table}


% BAK:

% \begin{table}[!h]
%   \centering
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{@{}lcccc@{}}
%     \toprule
%     \multirow{2}{*}{Method} & Appearance        & Temporal      & Structure             & Overall           \\
%                             &  Preservation     & Consistency   & Preservation          & Quality           \\
%     \midrule
%     Pose2Img                & 3.36              & 2.38          & 1.59                  & 2.01              \\
%     TPS                     & 2.03              & 2.10          & 1.18                  & 1.37              \\
%     DreamPose               & 2.78              & 1.94          & 2.27                  & 1.94              \\
%     DisCo                   & 2.27              & 2.32          & 1.45                  & 1.72              \\
%     Ours                    & \textbf{4.43}     & \textbf{4.21} & \textbf{4.05}         & \textbf{4.17}     \\
%     \bottomrule
%   \end{tabular}}
%   \caption{User study scores. The rating score is on a scale from one to five, where five is the highest score, and one is the lowest.}
%   \label{tab:userstudy}
% \end{table}

